ELLE: Efficient Lifelong Pre-training for Emerging Data

Current pre-trained language models (PLM) are typically trained with static data, ignoring that in real-world scenarios, streaming data of various sources may continuously grow. This requires PLMs to integrate the information from all the sources in a lifelong manner. Although this goal could be achieved by exhaustive pre-training on all the existing data, such a process is known to be computationally expensive. To this end, we propose ELLE, aiming at efficient lifelong pre-training for emerging data. Specifically, ELLE consists of (1) function preserved model expansion, which flexibly expands an existing PLM's width and depth to improve the efficiency of knowledge acquisition; and (2) pre-trained domain prompts, which disentangle the versatile knowledge learned during pre-training and stimulate the proper knowledge for downstream tasks. We experiment ELLE with streaming data from 5 domains on BERT and GPT. The results show the superiority of ELLE over various lifelong learning baselines in both pre-training efficiency and downstream performances. The codes are publicly available at https://github.com/thunlp/ELLE.

==> sections/table_big.tex <==
\begin{table*}[!t]
\small
\centering
\begin{tabu}{l@{~~~~}r@{~~~~}c@{~~~~}r@{~~~~}r@{~~~~}r@{~~~~}r@{~~~~}r@{~~~~}r@{~~~~}r@{~~~~}r}
\toprule
% \multicolumn{2}{c}{\textbf{Evaluated After}} & \multicolumn{2}{c}{Domain $1} & \multicolumn{2}{c}{Domain $2}    & \multicolumn{2}{c}{Domain $3}   & \multicolumn{2}{c}{Domain $4}   & \multicolumn{2}{c}{Domain $5}   \\ \hline
\multicolumn{1}{c}{\textbf{Domain}}          & \multicolumn{2}{c}{\textsc{WB}}       & \multicolumn{2}{c}{\textsc{Ns}}        & \multicolumn{2}{c}{\textsc{Rev}}     & \multicolumn{2}{c}{\textsc{Bio}}        & \multicolumn{2}{c}{\textsc{CS}}         \\ \hline
\multicolumn{1}{c}{\textbf{Metrics}}         & AP             & AP+       & AP            & AP+           & AP            & AP+          & AP            & AP+          & AP            & AP+          \\ \hline
\multicolumn{11}{l}{\textit{half pre-training wall time}} \\
MAS      & $7.96$          & - & $8.50$          & $6.22$          & $12.85$         & $18.88$         & $13.99$         & $17.52$         & $10.31$         & $10.22$         \\
ER       & $7.96$          & - & $7.12$          & $1.98$          & $7.11$          & $4.14$          & $6.83$          & $3.77$          & $6.53$          & $3.78$          \\
Logit-KD & $7.96$          & - & $7.72$          & $1.12$          & $7.27$          & $1.94$          & $7.17$          & $2.08$          & $7.06$          & $1.99$          \\
PNN      & $7.96$          & - & $6.75$          & $\textbf{0.00}$ & $5.53$          & $\textbf{0.00}$ & $5.09$          & $\textbf{0.00}$ & $5.03$          & $\textbf{0.00}$ \\
\ourmodel(ours)     & $\textbf{7.92}$ & - & $\textbf{6.05}$ & $0.26$          & $\textbf{5.21}$ & $1.04$          & $\textbf{4.83}$ & $0.96$          & $\textbf{4.42}$ & $0.68$   \\\hline
\multicolumn{11}{l}{\textit{smaller memory}} \\
MAS      & $7.96$            & -    & $8.08$          & $5.65$          & $13.44$         & $21.17$         & $13.87$         & $17.67$         & $9.91$          & $9.75$          \\
ER       & $7.96$            & -    & $6.99$          & $2.09$          & $7.15$          & $4.53$          & $6.86$          & $4.09$          & $6.49$          & $3.42$          \\
Logit-KD & $7.96$            & -    & $7.68$          & $1.15$          & $7.24$          & $2.06$          & $7.21$          & $2.27$          & $7.05$          & $2.16$          \\
PNN      & $7.96$            & -    & $6.52$          & $\textbf{0.00}$ & $5.29$          & $\textbf{0.00}$ & $4.84$          & $\textbf{0.00}$ & $4.76$          & $\textbf{0.00}$ \\
\ourmodel(ours)     & $\textbf{7.92}$   & -    & $\textbf{5.85}$ & $0.39$          & $\textbf{5.04}$ & $1.13$          & $\textbf{4.58}$ & $0.98$          & $\textbf{4.20}$ & $0.70$                 \\ \bottomrule       
\end{tabu}
\caption{Average perplexity (AP) and average increased perplexity ($\text{AP}^+$) of PLMs trained by different lifelong learning methods with half train wall time on Ns, Rev, Bio, CS domains and smaller memory containing $34$M tokens for each domains, respectively.  We evaluate the performance each time when PLMs finish training on one domain.}
\label{table:few_time_memory}
\end{table*}

\begin{table}[!t]
\centering
\small
\begin{tabu}{l@{~~~~}c@{~~~~}c@{~~~~}c@{~~~~}c@{~~~~}c@{~~~~}c}
\toprule
\textbf{Domain}        & \textsc{WB}        & \textsc{Ns}      & \textsc{Rev}    & \textsc{Bio}       & \textsc{CS}        & \textsc{AVG}       \\ \hline
\multicolumn{7}{l}{\textit{half pre-training wall time}} \\
MAS      & $76.7$          & $72.3$          & $61.6$          & $77.4$          & $64.3$          & $70.5$          \\
ER       & $78.0$          & $71.0$          & $61.1$          & $77.4$          & $65.8$          & $70.7$          \\
Logit-KD & $77.0$          & $72.6$          & $63.8$          & $76.2$          & $58.4$          & $69.6$          \\
PNN      & $76.0$          & $55.9$          & $62.6$          & $53.1$          & $28.0$          & $55.1$          \\
\ourmodel     & $\textbf{82.0}$ & $\textbf{78.4}$ & $\textbf{68.7}$ & $\textbf{81.7}$ & $\textbf{74.0}$ & $\textbf{77.0}$ \\ \hline
\multicolumn{7}{l}{\textit{smaller memory}} \\
MAS      & $77.1$                   & $73.7$                     & $60.7$                       & $77.5$                    & $68.2$                   & $71.5$                    \\
ER       & $77.9$                   & $72.0$                     & $61.5$                       & $76.3$                    & $63.6$                   & $70.3$                    \\
Logit-KD & $77.0$                   & $73.1$                     & $63.3$                       & $75.9$                    & $57.4$                   & $69.3$                    \\
PNN      & $76.0$                   & $64.9$                     & $64.2$                       & $55.1$                    & $30.5$                   & $58.1$                    \\
\ourmodel     & $\textbf{82.9}$          & $\textbf{80.5}$            & $\textbf{68.9}$              & $\textbf{82.6}$           & $\textbf{74.2}$          & $\textbf{77.8}$   \\ \hline
\end{tabu}
\caption{Final downstream performance (F1) of BERT on each domain after finishing pre-training on all domains with half train wall time on Ns, Rev, Bio, CS domains and smaller memory containing $34$M tokens for each domains, respectively. Experiments of \textsc{Ns} domain are repeated for $10$ times with different seeds and others are repeated for $5$ times. }
\label{table:downstream_few_time_memory}
\end{table}

==> sections/tables.tex <==
\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccc}
\tabucline[2pt]{-} 
\textbf{Evaluated After} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2}  & \multicolumn{2}{c}{Domain 3} & \multicolumn{2}{c}{Domain 4} & \multicolumn{2}{c}{Domain 5} \\ \hline
\textbf{Domain}          & \multicolumn{2}{c}{WB}       & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}   & \multicolumn{2}{c}{Bio}      & \multicolumn{2}{c}{CS}       \\ \hline
\textbf{Metrics}         & PPL               & $\text{PPL}^+$     & PPL           & $\text{PPL}^+$          & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        \\ \hline
Finetune                 & $7.96$              & /        & $8.03$          & $5.54$          & $13.52$          & $21.42$       & $13.86$          & 17.67       & 9.93           & 9.81        \\
EWC                      & 7.96              & /        & 8.09          & 5.65          & 13.4           & 20.98       & 13.92          & 17.75       & 9.94           & 9.82        \\
MAS                      & 7.96              & /        & 8.08          & 5.65          & 13.44          & 21.17       & 13.87          & 17.67       & 9.91           & 9.75        \\
GEM                      & 7.96              & /        & 8.82          & 6.72          & 13.31          & 20.06       & 14.73          & 18.89       & 10.56          & 10.58       \\
Replay                   & 7.96              & /        & 6.85          & 1.59          & 6.99           & 4.09        & 6.66           & 3.62        & 6.39           & 3.16        \\
Logit-KD                 & 7.96              & /        & 7.6           & 0.99          & 7.19           & 1.95        & 7.08           & 2.02        & 6.92           & 1.92        \\
PNN                      & 7.96              & /        & 6.52          & 0             & 5.29           & \textbf{0}  & 4.84           & \textbf{0}  & 4.76           & \textbf{0}  \\
Ours                     & \textbf{7.92}     & /        & \textbf{5.62} & \textbf{-0.2} & \textbf{4.81}  & 0.64        & \textbf{4.41}  & 0.64        & \textbf{4.06}  & 0.44       \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{Main Result: PPL }
\label{table:table1}
\end{table*}



\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccccc}
\tabucline[2pt]{-} 
\textbf{Domain}  & \multicolumn{2}{c}{WB}        & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}    & \multicolumn{2}{c}{BIO}       & \multicolumn{2}{c}{CS}        & \multicolumn{2}{c}{AVG}       \\ \hline
\textbf{Metircs} & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           \\\hline
Finetune         & $77.2$          & $22.45$         & $71.2$          & $17.78$         & $60.6$          & $13.25$         & $77.1$          & $4.93$          & $64.8$          & $3.70$          & $70.2$          & $9.93$          \\
EWC              & $77.4$          & $22.38$         & $70.6$          & $17.84$         & $61.6$          & $13.28$         & $77.5$          & $4.93$          & $59.6$          & $3.70$          & $69.4$          & $9.94$          \\
MAS              & $77.1$          & $22.39$         & $71.2$          & $17.68$         & $60.7$          & $13.15$         & $77.5$          & $4.93$          & $68.2$          & $3.70$          & $71.0$          & $9.91$          \\
GEM              & $76.6$          & $24.07$         & $71.4$          & $19.06$         & $61.5$          & $13.94$         & $76.9$          & $5.22$          & $67.5$          & $3.92$          & $70.7$          & $10.56$         \\
Replay           & $77.6$          & $13.36$         & $72.3$          & $8.85$          & $61.9$          & $5.49$          & $78.3$          & $4.37$          & $63.5$          & $3.77$          & $70.7$          & $6.39$          \\
Logit-KD         & $77.2$          & $12.33$         & $69.6$          & $8.67$          & $63.9$          & $5.60$          & $76.8$          & $5.03$          & $58.9$          & $5.24$          & $69.3$          & $6.92$          \\
PNN              & $76.0$          & $7.96$          & $64.8$          & $5.35$          & $64.2$          & $\mathbf{3.48}$ & $55.1$          & $3.71$          & $30.5$          & $4.43$          & $58.1$          & $4.76$          \\
\ourmodel             & $\mathbf{83.2}$ & $\mathbf{7.59}$ & $\mathbf{79.7}$ & $\mathbf{4.91}$ & $\mathbf{68.5}$ & $3.67$          & $\mathbf{82.9}$ & $\mathbf{2.89}$ & $\mathbf{72.7}$ & $\mathbf{2.77}$ & $\mathbf{77.4}$ & $\mathbf{4.06}$ \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{Main Result: downstream }
\label{table:table2}
\end{table*}

\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccc}
\tabucline[2pt]{-} 
\textbf{Evaluated After} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2}  & \multicolumn{2}{c}{Domain 3} & \multicolumn{2}{c}{Domain 4} & \multicolumn{2}{c}{Domain 5} \\ \hline
\textbf{Domain}          & \multicolumn{2}{c}{WB}       & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}   & \multicolumn{2}{c}{Bio}      & \multicolumn{2}{c}{CS}       \\ \hline
\textbf{Metrics}         & PPL               & $\text{PPL}^+$     & PPL           & $\text{PPL}^+$          & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        \\ \hline
Replay & 4.54          & / & 4.33          & 1.31          & 4.02          & 1.46          & 3.73          & 1.15          & 3.82          & 1.28          \\
Ours   & \textbf{4.52} & / & \textbf{3.89} & \textbf{0.47} & \textbf{3.61} & \textbf{0.75} & \textbf{3.66} & \textbf{0.97} & \textbf{3.29} & \textbf{0.54} \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{Larger Result: PPL }
\label{table:table3}
\end{table*}


\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccccc}
\tabucline[2pt]{-} 
\textbf{Domain}  & \multicolumn{2}{c}{WB}        & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}    & \multicolumn{2}{c}{BIO}       & \multicolumn{2}{c}{CS}        & \multicolumn{2}{c}{AVG}       \\ \hline
\textbf{Metircs} & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           \\\hline
Replay & 84.7          & 6.95          & 82.4          & 4.53          & 68.0          & 3.40          & 82.7          & 2.85          & 71.4          & 2.68          & 77.8          & 2.68          \\
Ours   & \textbf{86.3} & \textbf{5.47} & \textbf{90.4} & \textbf{3.67} & \textbf{70.5} & \textbf{3.01} & \textbf{84.2} & \textbf{2.54} & \textbf{73.8} & \textbf{2.52} & \textbf{81.0} & \textbf{2.52} \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{Larger Result: downstream }
\label{table:table4}
\end{table*}

\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccc}
\tabucline[2pt]{-} 
\textbf{Evaluated After} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2}  & \multicolumn{2}{c}{Domain 3} & \multicolumn{2}{c}{Domain 4} & \multicolumn{2}{c}{Domain 5} \\ \hline
\textbf{Domain}          & \multicolumn{2}{c}{WB}       & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}   & \multicolumn{2}{c}{Bio}      & \multicolumn{2}{c}{CS}       \\ \hline
\textbf{Metrics}         & PPL               & $\text{PPL}^+$     & PPL           & $\text{PPL}^+$          & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        \\ \hline
Finetune & 46.54          & / & 52.91          & 37.96         & 81.28          & 177.22        & 94.44          & 160.51        & 60.64          & 80.48         \\
MAS      & 46.54          & / & 53.12          & 38.44         & 81.23          & 177.20        & 93.21          & 157.93        & 60.62          & 80.28         \\
Replay   & 46.54          & / & 44.49          & 12.42         & 35.46          & 21.78         & 33.24          & 23.38         & 31.94          & 19.83         \\
Logit-KD & 46.54          & / & 48.93          & 5.41          & 37.60          & 9.97          & 34.60          & 11.74         & 33.67          & 11.19         \\
PNN      & 46.54          & / & 39.90          & \textbf{0.00} & 26.84          & \textbf{0.00} & \textbf{22.19} & \textbf{0.00} & 21.43          & \textbf{0.00} \\
ours     & \textbf{46.50} & / & \textbf{36.84} & 2.25          & \textbf{25.60} & 4.38          & 22.29          & 5.88          & \textbf{20.49} & 4.31          \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{GPT Result: PPL }
\label{table:table5}
\end{table*}

\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccc}
\tabucline[2pt]{-} 
\textbf{Evaluated After} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2}  & \multicolumn{2}{c}{Domain 3} & \multicolumn{2}{c}{Domain 4} & \multicolumn{2}{c}{Domain 5} \\ \hline
\textbf{Domain}          & \multicolumn{2}{c}{WB}       & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}   & \multicolumn{2}{c}{Bio}      & \multicolumn{2}{c}{CS}       \\ \hline
\textbf{Metrics}         & PPL               & $\text{PPL}^+$     & PPL           & $\text{PPL}^+$          & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        \\ \hline
ours                                   & \textbf{7.92} & \textbf{/} & \textbf{5.62} & \textbf{-0.20} & \textbf{4.81} & 0.64          & \textbf{4.41} & \textbf{0.64} & \textbf{4.06} & \textbf{0.44} \\
ours - DR                  & 7.92          & /          & 5.62          & -0.20          & 4.81          & \textbf{0.63} & 4.41          & 0.65          & 4.07          & 0.46          \\
ours - DR - prompt         & 7.96          & /          & 5.69          & -0.13          & 4.85          & 0.67          & 4.45          & 0.69          & 4.09          & 0.47          \\
ours - DR - prompt - noise & 7.96          & /          & 5.78          & 0.02           & 4.91          & 0.76          & 4.49          & 0.73          & 4.13          & 0.52    \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{Ablation Result 1: PPL }
\label{table:table6}
\end{table*}

\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccccc}
\tabucline[2pt]{-} 
\textbf{Domain}  & \multicolumn{2}{c}{WB}        & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}    & \multicolumn{2}{c}{BIO}       & \multicolumn{2}{c}{CS}        & \multicolumn{2}{c}{AVG}       \\ \hline
\textbf{Metircs} & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           & F1            & PPL           \\\hline
ours                                            & 83.2          & \textbf{7.59} & 79.7          & \textbf{4.91} & \textbf{68.5} & 3.67          & 82.9          & 2.89          & \textbf{72.7} & \textbf{2.77} & \textbf{77.4} & \textbf{4.06} \\
ours - DR                           & 83.0          & 7.68          & \textbf{80.0} & 4.96          & 68.3          & \textbf{3.65} & 82.4          & \textbf{2.88} & 70.7          & 2.78          & 76.9          & 4.07          \\
ours - DR - prompt                  & \textbf{83.5} & 7.73          & 77.3          & 5.03          & 66.9          & 3.66          & \textbf{83.3} & 2.88          & 70.6          & 2.78          & 76.3          & 4.09          \\
ours - DR - prompt - noise          & 83.4          & 7.86          & 75.6          & 5.11          & 67.4          & 3.67          & 82.4          & 2.91          & 71.5          & 2.81          & 76.1          & 4.13          \\
ours (finetune without prompt)                  & 82.9          & \textbf{7.59} & 77.8          & \textbf{4.91} & 65.5          & 3.67          & 82.5          & 2.89          & 71.2          & \textbf{2.77} & 76.0          & \textbf{4.06} \\
ours - DR (finetune without prompt) & 82.9          & 7.68          & 77.7          & 4.96          & 67.0          & \textbf{3.65} & 82.1          & \textbf{2.88} & 67.7          & 2.78          & 75.5          & 4.07           \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{Ablation Result: downstream }
\label{table:table7}
\end{table*}


\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccc}
\tabucline[2pt]{-} 
\textbf{Evaluated After} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2}  & \multicolumn{2}{c}{Domain 3} & \multicolumn{2}{c}{Domain 4} & \multicolumn{2}{c}{Domain 5} \\ \hline
\textbf{Domain}          & \multicolumn{2}{c}{WB}       & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}   & \multicolumn{2}{c}{Bio}      & \multicolumn{2}{c}{CS}       \\ \hline
\textbf{Metrics}         & PPL               & $\text{PPL}^+$     & PPL           & $\text{PPL}^+$          & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        \\ \hline
base                       & \textbf{7.96} & \textbf{/} & \textbf{5.78} & \textbf{0.02} & \textbf{4.91} & \textbf{0.76} & \textbf{4.49} & \textbf{0.73} & \textbf{4.13} & \textbf{0.52} \\
no recover                 & 7.96          & /          & 5.79          & 0.09          & 5.09          & 1.13          & 4.58          & 0.88          & 4.22          & 0.65          \\
add only layer             & 7.96          & /          & 5.81          & 0.03          & 5.49          & 1.43          & 5.16          & 1.32          & 4.79          & 0.94          \\
add only width             & 7.96          & /          & 6.23          & 0.78          & 5.34          & 1.42          & 4.98          & 1.20          & 4.48          & 0.89          \\
always add the first layer & 7.96          & /          & 5.80          & 0.04          & 4.98          & 0.87          & 4.55          & 0.81          & 4.22          & 0.63          \\
always add the last layer  & 7.96          & /          & 5.80          & 0.05          & 4.95          & 0.82          & 4.54          & 0.79          & 4.18          & 0.56        \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{Ablation Result 2: PPL }
\label{table:table8}
\end{table*}

\begin{table*}[!t]
\centering
\begin{tabu}{lcccccc}
\tabucline[2pt]{-} 
\textbf{Evaluated After} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2}  & \multicolumn{2}{c}{Domain 3}  \\ \hline
\textbf{Domain}          & \multicolumn{2}{c}{WB}       & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}  \\ \hline
\textbf{Metrics}         & PPL               & $\text{PPL}^+$     & PPL           & $\text{PPL}^+$          & PPL            & $\text{PPL}^+$ \\ \hline
add 0 layer and head per domain & \textbf{13.09} & /          & 8.99          & -0.49          & 8.24          & 2.80          \\
add 2 layer and head per domain & \textbf{13.09} & \textbf{/} & \textbf{8.28} & \textbf{-1.44} & \textbf{7.25} & \textbf{1.11} \\
add 4 layer and head per domain & \textbf{13.09} & /          & 8.62          & -0.95          & 7.53          & 1.30          \\
add 6 layer and head per domain & \textbf{13.09} & /          & 9.08          & -0.24          & 7.92          & 1.49     \\
\tabucline[2pt]{-} 
\end{tabu}
\caption{Ablation Result 3: PPL }
\label{table:table9}
\end{table*}

\begin{table*}[!t]
\centering
\begin{tabu}{lcccccccccc}
\tabucline[2pt]{-} 
\textbf{Evaluated After} & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2}  & \multicolumn{2}{c}{Domain 3} & \multicolumn{2}{c}{Domain 4} & \multicolumn{2}{c}{Domain 5} \\ \hline
\textbf{Domain}          & \multicolumn{2}{c}{WB}       & \multicolumn{2}{c}{News}      & \multicolumn{2}{c}{Review}   & \multicolumn{2}{c}{Bio}      & \multicolumn{2}{c}{CS}       \\ \hline
\textbf{Metrics}         & PPL               & $\text{PPL}^+$     & PPL           & $\text{PPL}^+$          & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        & PPL            & $\text{PPL}^+$        \\ \hline
ours                                   & \textbf{46.50} & \textbf{0.00} & \textbf{36.84} & \textbf{2.25} & \textbf{25.60} & \textbf{4.38} & \textbf{22.29} & \textbf{5.88} & \textbf{20.49} & \textbf{4.31} \\
ours - DR                  & 46.50          & 0.00          & 36.84          & 2.25          & 25.65          & 4.55          & 22.32          & 5.98          & 20.52          & 4.36          \\
ours - DR - prompt         & 46.54          & 0.00          & 37.01          & 2.49          & 25.80          & 4.87          & 22.51          & 6.40          & 20.71          & 4.70          \\
ours - DR - prompt - noise & 46.54          & 0.00          & 37.49          & 3.16          & 26.11          & 5.38          & 22.64          & 6.48          & 20.84          & 4.83                         \\ \tabucline[2pt]{-} 
\end{tabu}
\caption{GPT Ablation Result: PPL }
\label{table:table10}
\end{table*}

\begin{figure*}[!t]
\vfill
\centerline{
\begin{minipage}{0.24\textwidth}
    \begin{center}
    \includegraphics[width=\textwidth]{figs/main_avg_ppl.pdf}
    \end{center}
\end{minipage}
\hspace{0pt}
\begin{minipage}{0.24\textwidth}
\centerline{\includegraphics[width=\textwidth]{figs/main_avg_ppl_increased.pdf}}
\end{minipage}
\hspace{0pt}
\begin{minipage}{0.24\textwidth}
\centerline{\includegraphics[width=\textwidth]{figs/gpt_avg_ppl.pdf}}
\end{minipage}
\hspace{0pt}
\begin{minipage}{0.24\textwidth}
\centerline{\includegraphics[width=\textwidth]{figs/gpt_avg_ppl_increased.pdf}}
\end{minipage}
}
\caption{From left to right:.}
\label{fig:fig1}
\end{figure*}

\begin{table*}[]
\centering
\small
\begin{tabu}{lcccccccccc}
\toprule 
% \textbf{Evaluated After}   & \multicolumn{2}{c}{Domain 1} & \multicolumn{2}{c}{Domain 2}    & \multicolumn{2}{c}{Domain 3}   & \multicolumn{2}{c}{Domain 4}                & \multicolumn{2}{c}{Domain 5}                \\\hline
\textbf{Domain}            & \multicolumn{2}{c}{WB}       & \multicolumn{2}{c}{News}        & \multicolumn{2}{c}{Review}     & \multicolumn{2}{c}{Bio}                     & \multicolumn{2}{c}{CS}                      \\\hline
\textbf{Metrics}           & AP             & AP+       & AP            & AP+           & AP            & AP+          & AP                  & AP+                 & AP                  & AP+                 \\\hline
\multicolumn{11}{l}{\textbf{$\text{BERT}_\text{L6\_D384}$}}                 \\
\ourmodel                      & $\mathbf{7.92}$   & - & $\mathbf{5.62}$  & $\mathbf{-0.20}$ & $\mathbf{4.81}$  & $0.64$          & $\mathbf{4.41}$        & $\mathbf{0.64}$        & $\mathbf{4.06}$        & $\mathbf{0.44}$        \\
\ourmodel - DR                  & $\mathbf{7.92}$   & -          & $\mathbf{5.62}$  & $\mathbf{-0.20}$ & $\mathbf{4.81}$  & $\mathbf{0.63}$ & $\mathbf{4.41}$        & $0.65$                 & $4.07$                 & $0.46$                 \\
\ourmodel - DR - prompt         & $7.96$            & -          & $5.69$           & $-0.13$          & $4.85$           & $0.67$          & $4.45$                 & $0.69$                 & $4.09$                 & $0.47$                 \\
\ourmodel - DR - prompt - noise & $7.96$            & /          & $5.78$           & $0.02$           & $4.91$          & $0.76$          & $4.49$                & $0.73$                 & $4.13$                 & $0.52$                 \\\hline
Base                       & $\mathbf{7.96}$   & - & $\mathbf{5.78}$  & $\mathbf{0.02}$  & $\mathbf{4.91}$  & $\mathbf{0.76}$ & $\mathbf{4.49}$        & $\mathbf{0.73}$        & $\mathbf{4.13}$        & $\mathbf{0.52}$        \\
no FRW                 & $\mathbf{7.96}$            & -   & $5.79$           & $0.09$           & $5.09$           & $1.13$          & $4.58$                 & $0.88$                 & $4.22$                & $0.65$                 \\
expand depth only             & $\mathbf{7.96}$            & -          & $5.81$           & $0.03$           & $5.49$           & $1.43$          & $5.16$                 & $1.32$                 & $4.79$                 & $0.94$                 \\
expand width only       & $\mathbf{7.96}$            & -          & $6.23$           & $0.78$           & $5.34$           & $1.42$          & $4.98$                 & $1.20$                 & $4.48$                 & $0.89$                 \\
expand using the first layer only & $\mathbf{7.96}$            & -          & $5.80$           & $0.04$           & $4.98$           & $0.87$          & $4.55$                 & $0.81$                 & $4.22$                 & $0.63$                \\
expand using the last layer only  & $\mathbf{7.96}$            & -          & $5.80$           & $0.05$           & $4.95$           & $0.82$          & $4.54$                 & $0.79$                 & $4.18$                 & $0.56$                 \\\hline
expand 0 L \& H per domain      & $\mathbf{13.09}$           & -          & $8.99$           & $-0.49$          & $8.24$           & $2.80$          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
expand 2 L \& H per domain      & $\mathbf{13.09}$  & - & $\mathbf{8.28}$  & $\mathbf{-1.44}$ & $\mathbf{7.25}$  & $\mathbf{1.11}$ & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
expand 4 L \& H per domain      & $\mathbf{13.09}$           & -          & $8.62$          & $-0.95$          & $7.53$           & $1.30$          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
expand 6 L \& H per domain      & $\mathbf{13.09}$           & -          & $9.08$           & $-0.24$          & $7.92$           & $1.49$          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\\hline
\multicolumn{11}{l}{\textbf{$\text{GPT}_\text{L6\_D384}$}}                  \\
\ourmodel                       & $\mathbf{46.50}$  & -          & $\mathbf{36.84}$ & $\mathbf{2.25}$  & $\mathbf{25.60}$ & $\mathbf{4.38}$ & $\mathbf{22.29}$       & $\mathbf{5.88}$        & $\mathbf{20.49}$       & $\mathbf{4.31}$        \\
\ourmodel - DR                  & $\mathbf{46.50}$  & -          & $\mathbf{36.84}$ & $\mathbf{2.25}$  & $25.65$          & $4.55$          & $22.32$                & $5.98$                 & $20.52$                & $4.36$                 \\
\ourmodel - DR - prompt         & $46.54$           & -          & $37.01$          & $2.49$           & $25.80$          & $4.87$          & $22.51$                & $6.40$                 & $20.71$                & $4.70$                 \\
\ourmodel - DR - prompt - noise & $46.54$           & -          & $37.49$          & $3.16$           & $26.11$          & $5.38$          & $22.64$                & $6.48$                 & $20.84 $               & $4.83$                \\ \bottomrule
\end{tabu}
\caption{Average perplexity (AP) and average relative increased perplexity ($\text{AP}^+$) of language models pre-trained by our ELLE framework with different ablation operation. "DR", "FRW", and "L \& H" are shorts for "dynamic memory replay", "function recovering warmup", and "heads and layers", respectively.}
\label{table:table5}
\end{table*}

\begin{table*}[!t]
  \centering
  \small
    \begin{tabu}{cccccccc}
    \toprule 
            \multicolumn{1}{l}{$\textbf{Model}$}
          & \multicolumn{1}{l}{$n_{\text{params}}$} & \multicolumn{1}{l}{$n_{\text{layers}}$} & \multicolumn{1}{l}{$d_{\text{model}}$} & \multicolumn{1}{l}{$n_{\text{heads}}$} & \multicolumn{1}{l}{$d_{\text{FFN}}$} & \multicolumn{1}{l}{\text{lr ($\text{bs} = 2,048$)}}
          \\
    \hline
    \multicolumn{7}{l}{WE + FRW} \\
    $\mathcal{M}_{1}$ & $30.3$M      & $6$      & $384$      &  $6$     &   $1536$    &  $5.0\times10^{-4}$ \\
    $\mathcal{M}_{2}$ & $53.6$M      & $6$      & $576$      &  $9$     &   $2304$    &  $5.0\times10^{-4}$  \\
    $\mathcal{M}_{3}$ & $82.2$M      & $6$      & $768$      &  $12$     &   $3072$    &  $5.0\times10^{-4}$  \\
    $\mathcal{M}_{4}$ &  $104$M     & $6$   &  $896$ &  $14$ &  $3584$  &  $5.0\times10^{-4}$ \\
    $\mathcal{M}_{5}$ &  $129$M     & $6$   &  $1024$ &  $16$ &  $4096$  &  $5.0\times10^{-4}$  \\
    \hline
    \multicolumn{7}{l}{DE + FRW} \\
    $\mathcal{M}_{1}$ & $125$M      & $12$   &  $768$ &  $12$ &  $3072$  &  $5.0\times10^{-4}$ \\
    $\mathcal{M}_{2}$ & $51.6$M      & $18$   &  $768$ &  $12$ &  $3072$  &  $2.5\times10^{-4}$ \\
    $\mathcal{M}_{3}$ & $83.6$M      & $36$   &  $768$ &  $12$ &  $3072$  &  $2.5\times10^{-4}$ \\
    $\mathcal{M}_{4}$ & $105$M      & $48$   &  $768$ &  $12$ &  $3072$  &  $2.5\times10^{-4}$ \\
    $\mathcal{M}_{5}$ &  $126$M      & $60$   &  $768$ &  $12$ &  $3072$  &  $2.5\times10^{-4}$ \\
    \hline
    \multicolumn{7}{l}{WE + DE + FRW} \\
    $\mathcal{M}_{1}$ & $30.3$M      & $6$      & $384$      &  $6$     &   $1536$    &  $5.0\times10^{-4}$ \\
    $\mathcal{M}_{2}$ & $51.5$M      & $8$      & $512$      &  $8$     &   $2048$    &  $5.0\times10^{-4}$  \\
    $\mathcal{M}_{3}$ & $82.2$M      & $10$      & $640$      &  $10$     &   $2560$    &  $5.0\times10^{-4}$  \\
    $\mathcal{M}_{4}$ &  $102$M     & $11$   &  $704$ &  $11$ &  $2816$  &  $5.0\times10^{-4}$ \\
    $\mathcal{M}_{5}$ &  $125$M     & $12$   &  $768$ &  $12$ &  $3072$  &  $5.0\times10^{-4}$  \\
    \bottomrule
    \end{tabu}%
  \caption{Model architectures for WE + FRW, DE + FRW, WE + DE + FRW. We keep the total number of $\mathcal{M}_i$’s increased parameters for the above three strategies almost the same at each stage $i$. }
  \label{tab:arch_WE_DE}%
\end{table*}%

\begin{table*}[!t]
  \centering
  \small
    \begin{tabu}{ccccc}
    \toprule 
            \multicolumn{1}{l}{$\textbf{Model}$}
          & \multicolumn{1}{l}{Steps of FRW} 
          & \multicolumn{1}{l}{Steps of Training after FRW} 
          & \multicolumn{1}{l}{Ratio of Steps for lr Warmup} 
          & \multicolumn{1}{l}{Train Wall Time (s)} 
          \\
    \hline
    \multicolumn{5}{l}{\textit{Growing from} $\text{BERT}_\text{L6\_D384}$ \textit{to} $\text{BERT}_\text{L12\_D768}$} \\
    $\mathcal{M}_{1}$ & - & $62.5$k & $ 8\%$ & $6.0\times10^{4}$ \\
    $\mathcal{M}_{2}$ & $5$k & $20$k & $ 8\%$ & $2.4\times10^{4}$\\
    $\mathcal{M}_{3}$ & $5$k & $20$k  & $ 8\%$ & $5.0\times10^{4}$\\
    $\mathcal{M}_{4}$ & $5$k & $20$k & $ 8\%$ & $5.8\times10^{4}$\\
    $\mathcal{M}_{5}$ & $5$k & $20$k & $ 8\%$ & $6.8\times10^{4}$\\
    \hline
    \multicolumn{5}{l}{\textit{Growing from} $\text{BERT}_\text{L12\_D768}$ \textit{to} $\text{BERT}_\text{L24\_D1024}$} \\
    $\mathcal{M}_{1}$ & - & $62.5$k & $ 8\%$ & $1.9\times10^{5}$\\
    $\mathcal{M}_{2}$ & $1$k & $20$k  & $ 20\%$ & $6.5\times10^{4}$\\
    $\mathcal{M}_{3}$ & $1$k & $20$k  & $ 20\%$ & $1.4\times10^{5}$\\
    $\mathcal{M}_{4}$ &  $1$k & $20$k & $ 20\%$ & $1.7\times10^{5}$ \\
    $\mathcal{M}_{5}$ &  $1$k & $20$k & $ 20\%$ & $2.2\times10^{5}$  \\
    \hline
    \multicolumn{5}{l}{\textit{Growing from} $\text{GPT}_\text{L6\_D384}$ \textit{to} $\text{GPT}_\text{L12\_D768}$} \\
    $\mathcal{M}_{1}$ &  - & $62.5$k  & $ 16\%$ & $6.7\times10^{4}$ \\
    $\mathcal{M}_{2}$ & $5$k & $20$k  & $ 16\%$ & $3.9\times10^{4}$\\
    $\mathcal{M}_{3}$ & $5$k & $20$k  & $ 16\%$ & $5.6\times10^{4}$\\
    $\mathcal{M}_{4}$ &  $5$k & $20$k & $ 16\%$ & $ 6.8\times10^{4}$\\
    $\mathcal{M}_{5}$ &  $5$k & $20$k & $ 16\%$ & $7.8\times10^{4}$ \\
    \bottomrule
    \end{tabu}%
  \caption{Steps of FRW, steps of training after FRW, the ratio of steps for learning rate warmup (for both FRW and pre-training), and train wall time on each domain for all the models we used in this paper. The total train wall time consumed by $\text{BERT}_\text{L6\_D384}$, $\text{BERT}_\text{L12\_D768}$ and $\text{GPT}_\text{L6\_D384}$ are $2.57 \times 10^5$ seconds, $7.79 \times 10^5$ seconds, and $3.08 \times 10^5$ seconds in total, respectively.}
  \label{table:steps}%
\end{table*}%
